Injecting Text and Cross-lingual Supervision in Few-shot Learning from Self-Supervised Models

Self-supervised model pre-training has recently garnered significant interest, but relatively few efforts have explored using additional resources in fine-tuning these models. We demonstrate how universal phoneset acoustic models can leverage cross-lingual supervision to improve transfer of pretrained self-supervised representations to new languages. We also show how target-language text can be used to enable and improve fine-tuning with the lattice-free maximum mutual information (LF-MMI) objective. In three low-resource languages these techniques greatly improved few-shot learning performance.

==> figures/phonelm_order_vs_weight.tex <==
\begin{tikzpicture}
\begin{axis}[
    xlabel=n-gram order,
    ylabel=WER \%,
    height=4cm, width=8cm,
    ymin=64.5,
    ymax=70,
    xmin=0,
    xmax=4,
    legend columns=2,
    legend style={at={(0.8,1.0)}},
    x label style={at={(axis description cs:0.5,-0.15)},anchor=north},
    y label style={at={(axis description cs:-0.08,.5)},anchor=south},
    ]
\addplot[mark=*,blue] plot coordinates {
    (0, 81.9)
    (1, 66.2)
    (2, 65.2)
    (3, 68.2)
    (4, 74.7)
};
\addlegendentry{$\alpha=0.0$}
% \addplot[mark=*,blue] plot coordinates {
%     (0, 81.9)
%     (1, 65.7)
%     (2, 65.3)
%     (3, 66.7)
%     (4, 67.6)
% };
% \addlegendentry{$\alpha=0.05$}
\addplot[dashed, mark=*,red] plot coordinates {
    (0, 81.9)
    (1, 66.1)
    (2, 65.0)
    (3, 66.3)
    (4, 67.6)
};
\addlegendentry{$\alpha=0.1$}
\addplot[dotted, mark=*, olive] plot coordinates {
    (0, 81.9)
    (1, 66.3)
    (2, 65.1)
    (3, 66.1)
    (4, 66.8)
};
\addlegendentry{$\alpha=0.2$}
\addplot[mark=*,blue] plot coordinates {
    (0, 81.9)
    (1, 65.9)
    (2, 65.2)
    (3, 66.3)
    (4, 67.2)
};
\addlegendentry{$\alpha=0.5$}
\end{axis}
\end{tikzpicture}

==> tables/LFMMI_Denom.tex <==
\begin{tabular}{@{}l|ll|ll|ll|ll|ll|ll|@{}}
\cmidrule(l){2-13}
                                            & \multicolumn{6}{c|}{200}                                                       & \multicolumn{6}{c|}{LLP}                                                       \\ \cmidrule(l){2-13} 
\multicolumn{1}{c|}{}                       & \multicolumn{2}{c|}{pus} & \multicolumn{2}{c|}{hat} & \multicolumn{2}{c|}{kat} & \multicolumn{2}{c|}{pus} & \multicolumn{2}{c|}{hat} & \multicolumn{2}{c|}{kat} \\ \cmidrule(l){2-13} 
\multicolumn{1}{c|}{Initial Model}          & Den        & Den2        & Den        & Den2        & Den        & Den2        & Den        & Den2        & Den        & Den2        & Den        & Den2        \\ \midrule
\multicolumn{1}{|l|}{Random}                &            &             &            &             &            &             &            &             &   57.7         &             &            &             \\
\multicolumn{1}{|l|}{XL-WRN Multi-phoneset} &            &             &            &             &            &             &            &             &            &             &            &             \\
\multicolumn{1}{|l|}{XL-WRN Mono-phoneset}  &            &             &            &             &            &             &            &             &    52.3        &      52.8      &             \\
\multicolumn{1}{|l|}{LV60}                  &            &             &            &             &            &             &            &             &    50.3        &     50.6        &            &             \\
\multicolumn{1}{|l|}{VoxPopuli 100k-Large}  &            &             &            &             &            &             &            &             &    48.0       &     47.9        &            &             \\
\multicolumn{1}{|l|}{XLSR-53}               &            &             &            &             &            &             &            &             &    45.3        &     45.2        &            &             \\ \bottomrule
\end{tabular}

==> tables/Multilingual_Pretraining_Strategies.tex <==
\begin{tabular}{@{}lllccccccccc@{}}
                                                      &              &                                      & \multicolumn{9}{c}{Fine Tuning}                                                                                                                                                                                                              \\ \cmidrule(l){4-12} 
                                                      & \multicolumn{2}{c|}{Pretraining Data (hr)}                  & \multicolumn{3}{c|}{200 Utts}                                              & \multicolumn{3}{c|}{LLP}                                             & \multicolumn{3}{c}{FLP}                                            \\ \midrule
\multicolumn{1}{c|}{Model}                    & Labeled & \multicolumn{1}{l|}{Unlabeled} & \multicolumn{1}{l}{pus} & \multicolumn{1}{l}{hat} & \multicolumn{1}{l|}{kat} & \multicolumn{1}{l}{pus} & \multicolumn{1}{l}{hat} & \multicolumn{1}{l|}{kat} & \multicolumn{1}{l}{pus} & \multicolumn{1}{l}{hat} & \multicolumn{1}{l}{kat} \\ \midrule
\multicolumn{1}{l|}{CTC-BLSTM Random \cite{dalmia2018sequence}}                           & 0            & \multicolumn{1}{l|}{0}               & -                       & -                       & \multicolumn{1}{c|}{-}   & -                       & -                       & \multicolumn{1}{c|}{-}   & -                       & 49.0                      & -                       \\
\multicolumn{1}{l|}{CTC-BLSTM Multi-Lingual\cite{dalmia2018sequence}}                           & 0.5k            & \multicolumn{1}{l|}{0}               & -                       & -                       & \multicolumn{1}{c|}{-}   & -                       & -                       & \multicolumn{1}{c|}{-}   & -                       & 44.3                      & -                       \\ 
\multicolumn{1}{l|}{MLBNFeats-MPE-LSTM-RNN\cite{golik20172016}}                           & 1.8k            & \multicolumn{1}{l|}{0}               & -                       & -                       & \multicolumn{1}{c|}{-}   & -                       & -                       & \multicolumn{1}{c|}{-}   & 47.1                       & -                   & -                       \\
\multicolumn{1}{l|}{CTC-BLSTM Multi-Lingual Adversarial \cite{yi2019language}}                           & 0.2k            & \multicolumn{1}{l|}{0}               & -                       & -                       & \multicolumn{1}{c|}{-}   & -                       & -                       & \multicolumn{1}{c|}{-}   & 43.4                       & -                   & -                       \\
\multicolumn{1}{l|}{Multi-Lingual lf-MMI BLSTM \cite{alumae20172016}}                           & 0            & \multicolumn{1}{l|}{2.4k}               & -                       & -                       & \multicolumn{1}{c|}{-}   & -                       & -                       & \multicolumn{1}{c|}{-}   & -                      & -                   & 35.1                      \\
\multicolumn{1}{l|}{XLSR-53 \cite{conneau2020unsupervised}}                           & 0            & \multicolumn{1}{l|}{56k}               & -                       & -                       & \multicolumn{1}{c|}{-}   & -                       & -                       & \multicolumn{1}{c|}{-}   & -                      & -                   & 31.1                      \\
\midrule
\multicolumn{1}{l|}{Random}                           & 0            & \multicolumn{1}{l|}{0}               & -                       & -                       & \multicolumn{1}{c|}{-}   & 61.1                       & 57.7                       & \multicolumn{1}{c|}{57.6}   & 50.1                       & 46.6                       & 49.5                       \\
\multicolumn{1}{l|}{XL-WRN Mono-phoneset}  & 1.2k         & \multicolumn{1}{l|}{0}               & -                       & -                       & \multicolumn{1}{c|}{-}   & -                       & 52.3                       & \multicolumn{1}{c|}{-}   & -                       & 43.3                       & -                       \\
\multicolumn{1}{l|}{LV60}                             & 0            & \multicolumn{1}{l|}{60k}             & -                       & -                       & \multicolumn{1}{c|}{-}   & 50.3                       & 50.3                       & \multicolumn{1}{c|}{50.5}   & 42.8                       & 40.8                       & 43.1                       \\
\multicolumn{1}{l|}{Large-Robust}                     & 0            & \multicolumn{1}{l|}{63k}             & -                       & -                       & \multicolumn{1}{c|}{-}   & 49.5                       & 49.1                       & \multicolumn{1}{c|}{48.7}   & 41.8                       & 40.4                       & 42.2                       \\
\multicolumn{1}{l|}{VoxPopuli-100k-Large}             & 0            & \multicolumn{1}{l|}{100k}            & -                       & -                       & \multicolumn{1}{c|}{-}   & 48.9                       & 48.0                      & \multicolumn{1}{c|}{47.9}   & 41.1                       & 39.3                       & 41.5                       \\
\multicolumn{1}{l|}{XLSR-53}                          & 0            & \multicolumn{1}{l|}{56k}             & -                       & -                       & \multicolumn{1}{c|}{-}   & 45.5                       & 45.3                       & \multicolumn{1}{c|}{45.1}   & 39.4                       & 37.7                       & 40.0                       \\
\multicolumn{1}{l|}{\quad + expanded vocab.}                          & 0            & \multicolumn{1}{l|}{56k}             & -                       & -                       & \multicolumn{1}{c|}{-}   & 45.1                        & -                       & \multicolumn{1}{c|}{-}   & 38.8                       & 36.9                        & 32.2                       \\
 \midrule
\multicolumn{1}{l|}{Wav2Vec2 Random}                      & 0            & \multicolumn{1}{l|}{60k}             & -                       & -                       & \multicolumn{1}{c|}{-}   & -                       & -                       & \multicolumn{1}{c|}{-}   & -                       & -                       & -                       \\
\multicolumn{1}{l|}{XLSR-53}                      & 0            & \multicolumn{1}{l|}{0.96k}             & -                       & -                       & \multicolumn{1}{c|}{-}   & -                       & -                       & \multicolumn{1}{c|}{-}   & -                       & -                       & -                       \\ 
\multicolumn{1}{l|}{XLSR-53 + Multi-phoneset}                      & 0            & \multicolumn{1}{l|}{2.16k}             & -                       & -                       & \multicolumn{1}{c|}{-}   & -                       & -                       & \multicolumn{1}{c|}{-}   & -                       & -                       & -                       \\
\bottomrule
\end{tabular}

==> tables/adaptation_techniques_201.tex <==
\begin{tabular}{@{}ccccccc@{}}
\toprule
\multicolumn{1}{l}{}                       & \multicolumn{6}{c}{\textbf{Adaptation Method}}                                                                                                                                                                                                                                                                           \\ \midrule
\multicolumn{1}{l}{\textbf{\# Utts}} & \multicolumn{1}{l}{Multi-500-LP} & \multicolumn{1}{l}{Multi-500} & \multicolumn{1}{l}{Multi-3500} & \multicolumn{1}{l}{Mono} & \multicolumn{1}{l}{Mono-full-den} & \multicolumn{1}{l}{Scratch}\\
100                                        & 75.3                                                                                  & 74.2                                                                            & \textbf{74.1}                               & 89.2                           & 86.5                                        & -\\
200                                        & 71.9                                                                                   & 71.2                                                                          & \textbf{70.3}                               & 80.9                           & 77.8                                     & -   \\
400                                        & 70.6                                                                                 & \textbf{69.1}                                                                    & 69.7                                        & 72.8                           & 71.1                                       & - \\
800                                        & 68                                                                                   & \textbf{66.7}                                                                   & 67                                          & 67.9                           & 67.3                                       & - \\
1600                                       & 65.2                                                                                     & 64.4                                                                             & 62.8                                        & 62                             & \textbf{61.9}                             & -  \\
3200                                       & 63.9                                                                                   & 62.6                                                                             & 61.4                                        & 59.7                           & \textbf{59.5}                            & -   \\
6400                                       & 62.6                                                                                    & 61.9                                                                              & 59.8                                        & 57.7                           & \textbf{57.4}                            & -   \\
10000                                      & 60.1                                                                                   & 59.6                                                                             & 56.2                                        & 54.2                           & \textbf{54.2}                            & 59.2   \\ \bottomrule
\end{tabular}


==> tables/wav2vec_hyperparam_tuning.tex <==
\begin{tabular}{@{}l|cc@{}}
\toprule
                                      & \multicolumn{1}{l}{201-Haitian tune} & \multicolumn{1}{l}{201-Haitian Dev10h} \\ \midrule
Vox Populi Wav2Vec2 v.1 ds 640x             & 51.0                                 & -                                      \\
XLSR-53 Wav2Vec2 v.1 ds 640x                 & 48.3                                 & -                                      \\
Vox Populi Wav2Vec2 v.1 Z-norm ds 640x   & 49.4                                 & -                                      \\
XLSR-53 Wav2Vec2 v2. Z-norm no time mask ds 640x & 48.2 & - \\
XLSR-53 Wav2Vec2 v2. Z-norm ds 320x & 48.2 & - \\
XLSR-53 Wav2Vec2 v.1 Z-norm ds 640x         & 48.0                                 & -                                      \\
XLSR-53 Wav2Vec2 v.2 Z-norm ds 640x         & 48.0                                 & -                                      \\
XLSR-53 Wav2Vec2 v.2 Z-norm ds 640x Schedule 2 Freeze-FE & 46.7 & - \\
XLSR-53 Wav2Vec2 v.2 Z-norm ds 640x Schedule 2 & 46.2 & - \\
\bottomrule
\end{tabular}
